UR-FUNNY: A Multimodal Language Dataset for Understanding Humor

Humor is a unique and creative communicative behavior displayed during social interactions. It is produced in a multimodal manner, through the usage of words (text), gestures (vision) and prosodic cues (acoustic). Understanding humor from these three modalities falls within boundaries of multimodal language; a recent research trend in natural language processing that models natural language as it happens in face-to-face communication. Although humor detection is an established research area in NLP, in a multimodal context it is an understudied area. This paper presents a diverse multimodal dataset, called UR-FUNNY, to open the door to understanding multimodal language used in expressing humor. The dataset and accompanying studies, present a framework in multimodal humor detection for the natural language processing community. UR-FUNNY is publicly available for research.

==> figures/Omission_f1_score/omission.tex <==
\begin{figure*}
\includegraphics[width=0.5\linewidth]{acl2019-latex/figures/Omission_f1_score/f1_score_after_omit.pdf}
\caption{F-1 score after omitting features}
\label{fig:f1_omit}
\end{figure*}

==> figures/humor_model_old/humor_model.tex <==
\begin{figure}
\includegraphics[width=1.1\linewidth]{unimodal.pdf}
\caption{proposed model}
\label{fig:unimodal}
\end{figure}

==> tables/drop_feature.tex <==
\begin{table}[t!]
\begin{center}
\small
\begin{tabular}{l|r|s|}
\hline F1-Score & Accuracy & Omitted Feature\\
\hline 64.37 & 64.13 & mcep \\ 
\hline 64.43 & 63.8 & upper face \\
\hline 64.46 & 64.32 & formant\\
\hline 64.51 & 64.19 & fear \\
\hline 64.51 & 64.32 & peak slope \\
\hline 64.54 & 64.19 & lower face\\
\hline 64.54 & 64.19 & pitch\\ 
\hline 64.60 & 64.50 & surprise \\ 
\hline 64.66 & 64.29 & quotient \\
\hline 64.70 & 64.70 & anger \\
\hline 64.71 & 64.47 & harmonic \\ 
\hline 64.75 & 64.65 & shape-parameters \\ 
\hline 64.78 & 64.26 & pdm \\
\hline 64.80 & 64.70 & happiness\\
\hline 64.87 & 64.38 & pdd \\
\hline 65.30 & 65.23 & sadness\\

\hline
\end{tabular}
\end{center}
\caption{\label{summary} F-1 score and accuracy after omitting a particular feature during training. The entries are sorted according to increasing values of F-1 score and accuracy. The earlier rows have more impact on predicting humor instances.}
\end{table}

==> tables/featuresubsets.tex <==
\begin{table}[t!]
\begin{center}
\small
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{l}
\hline 
\textbf{Visual Subsets} \\
Upper Face : Action Units- 01,02,04,05,06,07,45\\
Lower Face : Action Units- 09,10,12,14,15,17,20,23,25,26\\
Happiness  : Action Units- 06,12 \\
Sadness :  Action Units- 01,04,15\\
Surprise : Action Units- 01,02,05,26\\
Anger : Action Units- 04,05,07,23 \\
Disgust : Action Units- 09,15,17\\
Fear : Action Units - 01,02,04,05,07,20,26\\\hline
\textbf{Acoustic Subsets} \\
Mel Cepstral Coefficient : MCEP 0-24 \\ 
Harmonic Phase Distortion Mean :  HMPDM 0-24 \\
Harmonic Phase Distortion Deviation : HMPDD 0-12 \\
Formant : F 1-5 \\
Peak Slope : peakslope \\ 
Pitch : f0 \\
Harmonic : H1H2 \\
Quasi Open Quotient : QOQ \\
\hline
\end{tabular}
\end{center}
\caption{ Features Set Experiment}
\label{table:fetaure_experiment}
\end{table}
